Redesigning graph filter-based GNNs to relax the homophily assumption

Graph neural networks (GNNs) have become a workhorse approach for learning from data defined over irregular domains, typically by implicitly assuming that the data structure is represented by a homophilic graph. However, recent works have revealed that many relevant applications involve heterophilic data where the performance of GNNs can be notably compromised. To address this challenge, we present a simple yet effective architecture designed to mitigate the limitations of the homophily assumption. The proposed architecture reinterprets the role of graph filters in convolutional GNNs, resulting in a more general architecture while incorporating a stronger inductive bias than GNNs based on filter banks. The proposed convolutional layer enhances the expressive capacity of the architecture enabling it to learn from both homophilic and heterophilic data and preventing the issue of oversmoothing. From a theoretical standpoint, we show that the proposed architecture is permutation equivariant. Finally, we show that the proposed GNNs compares favorably relative to several state-of-the-art baselines in both homophilic and heterophilic datasets, showcasing its promising potential.

==> figs/freq_responses.tex <==
\begin{tikzpicture}[baseline,scale=1]

\pgfplotstableread{data/20240906-1202-CoraGraphDataset-filter_freq.csv}\errtable


\begin{axis}[
    xlabel={(b) Eigenvalues},
    %xmin=1,
    %xmax=1060,
    %xtick = {1, 250, 500, 750, 1000},
    %ylabel={},
    %ymin = 0,
    %ymax = .35,
    %ytick = {0, .1, ..., .51},
    grid style=densely dashed,
    grid=both,
    legend style={
        at={(0, 1)},
        anchor=north west},
    legend columns=1,
    width=127,
    height=130,
    ]
    
    % Plot Confident interval
    \addplot[blue, solid] table [x=AFGNN-normH-xax, y=CoraGraphDataset-AFGNN-normH-filterfreqs] {\errtable};

    % Add dashed vertical lines

    %\legend{Err, Cum Err}
\end{axis}
\end{tikzpicture}

==> figs/test.tex <==

\begin{tikzpicture}[baseline,scale=.75,trim axis left, trim axis right]

\pgfmathsetmacro{\initmarksize}{3.5}

\pgfplotsset{colormap={CM}{
    rgb255=(54, 75, 154)
    rgb255=(74, 123, 183)
    rgb255=(110, 166, 205)
    rgb255=(152, 202, 225)
    rgb255=(194, 228, 239)
    rgb255=(234, 236, 204)
    rgb255=(254, 218, 139)
    rgb255=(253, 179, 102)
    rgb255=(246, 126, 75)
    rgb255=(221, 61, 45)
    rgb255=(165, 0, 38)
}}

\begin{loglogaxis}[
        view={0}{90},
        title=Error, 
        % scale only axis,
        xlabel={(a) Bias penalty weight $\mu_2$},
        ylabel={Sparsity penalty weight $\mu_1$},
        tick style={draw=none},
        ylabel shift = {-1.5},
        width=200,
        height=200,
        label style={font=\small},
        tick label style={font=\small},
        colorbar
    ]
    \addplot3[surf, mesh/rows=12] 
        table[x=mu2,y=mu1,z=frob_fair, col sep=comma]
        {data/hyperparam_table.csv};
\end{loglogaxis}

\end{tikzpicture}
